Entity-Based Knowledge Conflicts in Question Answering

Knowledge-dependent tasks typically use two sources of knowledge: parametric, learned at training time, and contextual, given as a passage at inference time. To understand how models use these sources together, we formalize the problem of knowledge conflicts, where the contextual information contradicts the learned information. Analyzing the behaviour of popular models, we measure their over-reliance on memorized information (the cause of hallucinations), and uncover important factors that exacerbate this behaviour. Lastly, we propose a simple method to mitigate over-reliance on parametric knowledge, which minimizes hallucination, and improves out-of-distribution generalization by 4%-7%. Our findings demonstrate the importance for practitioners to evaluate model tendency to hallucinate rather than read, and show that our mitigation strategy encourages generalization to evolving information (i.e., time-dependent queries). To encourage these practices, we have released our framework for generating knowledge conflicts.

==> sections/1-introduction.tex <==
\section{Introduction}
\respace

Progress in question answering (QA) has been steadily driven by new datasets \cite{Rajpurkar2016SQuAD10} and better models \citep{Seo2017BidirectionalAF}. \erik{cite two of each?}
Recent progress has been boosted \erik{pv awkward} by the use of large language models which first pre-train on enormous amounts of unlabeled data before being fine-tuned as a question answering system \citep{Peters2018DeepCW, Devlin2019BERTPO}.
As a testament to the abilities of these language models, it is well established that some are able to achieve decent performance \erik{what is performance? try to replace with accuracy, some metric...} relying only on their own parametric knowledge \erik{probably define outside of the paranthetical, since it's important}(\textit{i.e.}, their weights), without access to documents to reason over \citep{Brown2020LanguageMA}.

The use of pre-trained language models as QA systems \erik{could be clean to conciesly state how they're used: language models respond to questions by XXX} has raised questions about the interplay between the internal parametric knowledge learned during pre-training and fine-tuning and the external contextual knowledge provided in the form of documents \ej{how is this external knowledge incorporated? up until now we've just been talking about language models?}
In an idealized situation, QA systems should produce an answer that is grounded in the context and rely on parametric knowledge only when appropriate. \erik{when is appropriate?}
However, recent work has demonstrated that pre-trained language models have a penchant to hallucinate answers sourced from their parametric memory, completely ignoring the context \citep{Krishna2021HurdlesTP}.
This has practical ramifications as models which are insensitive to contextual information will struggle to perform in real-world situations where information changes over time \ej{probably don't need to narrow focus to time} \citep{Shuster2021RetrievalAR}.
While these problems are known, it is unclear which factors (\textit{e.g.} model size, seen vs unseen questions \ej{what is a seen question}) contribute to a model's tendency to overly rely on a particular form of knowledge.
\ej{Overall, I feel like these first two paragraphs get into the weeds to quickly. It would be nice to know 1. concretely, how a system leverages both parameters and documents to answer a question (that way people can think about what goes wrong), 2. pros/cons (especially the pros) of relying on parameters to answer questions, before going deeper}
\ej{Also, whenever you use a somewhat vernacular term (e.g. "parametric knowledge", "seen questions", ...) define it first.}

% Motivating Figure
\begin{figure}[t!]
    \begin{framed}
        \small \textbf{Question:} who did US fight in world war 1?\\
        
        \textbf{Original Context:} The United States declared war on \textbf{\textcolor{red}{Germany}} on April 6, 1917, over 2 years after World War I started. A ceasefire and Armistice was declared on November 11, 1918 \ldots \\
        \textbf{Original Answer:} \textbf{\textcolor{red}{Germany}} \\
        \textbf{Prediction:} \textbf{\textcolor{red}{Germany}} \\
        
        \textbf{Substituted Context:} The United States declared war on \textbf{\textcolor[RGB]{30,111,50}{Taiwan}} on April 6, 1917, over 2 years after World War I started. A ceasefire and Armistice was declared on November 11, 1918 \ldots \\
        \textbf{Substituted Answer:} \textbf{\textcolor[RGB]{30,111,50}{Taiwan}} \\
        \textbf{Prediction:} \textbf{\textcolor{red}{Germany}}
    \end{framed}
    
    \caption{\textbf{A knowledge conflict generated by our substitution framework.} A generative QA model predicts the original answer \textbf{\textcolor{red}{Germany}} despite the substituted context supporting \textbf{\textcolor[RGB]{30,111,50}{Taiwan}}.}
    \label{fig:introduction:example}
    \vspace*{-.4cm}
\end{figure}  
\respace

The objective of this work is to understand how systems balance parametric and contextual knowledge by studying knowledge conflicts: situations where the contextual knowledge contradicts with knowledge learned during pre-training or fine-tuning. \ej{nice}
Because the space of knowledge conflicts is broad, we restrict ourselves to the space of \textit{entity-based} conflicts. \ej{define}
We create an automated framework that first identifies QA instances where the answer is identified as a named entity, then substitute all instances of the entity in the gold document with an alternate entity, thus changing what the answer should be (Fig. \ref{fig:introduction:example}).
Our framework is flexible and allows for alternate entities to be mined from various sources, such as the corpus of entities from the original dataset and from knowledge graphs like Wikidata \citep{Vrandecic2014WikidataAF}. \ej{why is this important? i'd either contextualize why or cut}

We use our automated framework to create substituted instances for Natural Questions \citep{Kwiatkowski2019NaturalQA} and NewsQA \citep{Trischler2017NewsQAAM}.
Using these substituted documents, we evaluate several popular models under a variety of ablations, such as model size, training with gold vs retrieved documents, and the degree to which the substitution set is out-of-domain from the training set.
When isolating these factors, we discover several interesting phenomenon that contribute to over-reliance on parametric knowledge. \ej{cut, get directly to findings}
For instance, training with retrieved documents instead of gold documents greatly increases the chance of the original entity as an answer, even when the substituted document only contains the substituted entity.
Additionally, \ej{we find that}the larger the model, the greater the proclivity to rely on parametric knowledge.
As a mitigation strategy, we demonstrate that training with the substituted document not only reduces memorization from \textcolor{red}{XXX} to \textcolor{red}{XXX} on the substituted documents, but also increases generalization by \textcolor{red}{XXX} on original documents of OOD data. \ej{OOD data feels like an afterthought, but people will find it interesting. could you motivate?}


==> sections/5-discussion.tex <==
\section{Discussion}
\label{discussion}

==> sections/old_introduction.tex <==
\section{Introduction}

Modern natural language tasks, such as open-retrieval question answering (QA) and fact verification (FV), pose problems that require more than local reasoning over a textual input.
These can also require expansive ``world knowledge'', common sense, and a broad understanding of informational topics.

State-of-the-art approaches to information-seeking tasks typically follow a retrieve-and-read setup \citep{chen2017reading}, where the knowledge retriever sources a subset of relevant information, given to the reader to reason an appropriate answer.
A common implicit assumption is the reader should trust and not contradict the retrieved knowledge.
However, in practice this expectation is not well enforced, with generative reader models having been observed to hallucinate answers sourced from their parametric memory or learned biases \citep{krishna2021hurdles}.

In this sense, there are two sources of knowledge contributing to model inference, with what remains an ambiguous and opaque division of labour.
The first is the implicit parametric knowledge, instilled by large scale pre-training and fine-tuning \citep{petroni2019language}. 
The second is external knowledge, usually sourced as passages of text from the retriever model \citep{fisch2019mrqa, Thorne19FEVER2}.

In this work, we pose the question: how does the model behave when faced with contradictions in these two sources of knowledge?
We test this by modifying contextual knowledge given to question answering models, such that the retrieved passages imply a different answer than the training data (pre-training or fine-tuning).
Further, we find models behave radically differently in these tests, depending on a number of factors, including training methodology, model size, model type, domain similarity, and characteristics of the substituted answer.

% In doing so, we empirically examine how these knowledge sources affect model inference, as well as the implications for assumptions regarding the desired relationship between retriever and reader.

To our knowledge, no detailed examination of this phenomena has been conducted, but it is well motivated with relevant implications for three timely areas of investigation.

\begin{enumerate}\itemsep0em
  \item Large neural models have been shown to systematically parrot training and pre-training data, learning to \textit{memorize} rather than reason or \textit{generalize} \citep{lewis2020question, 10.1145/3442188.3445922}.
  \item Recent QA research has focused primarily on static knowledge representations, i.e. specific Wikipedia dumps, and fails to factor in evolving knowledge and time-dependent queries. This problem is observed in Appendix C of \citep{guu2020realm}.
  \item Large parametric knowledge representations are often non-robust, demonstrating sensitivity to knowledge poisoning or being fooled by information attacks \citep{wallace2019universal, wallace2020customizing}.
\end{enumerate}

Together, these observations suggest vulnerabilities in knowledge usage may inhibit modern system's capacity to generalize, model time-dependent phenomena, or adequately defend against adversarial inputs.

To understand model behaviour, we isolate common answer types in Natural Questions \citep{kwiatkowski2019natural} and substitute for answers of the same type, sourced from WikiData.\footnote{Wikidata is a collaboratively edited open knowledge
graph: \url{https://www.wikidata.org/}.}
Our contributions include:
\begin{itemize}\itemsep0em
  \item \textbf{Substitution Framework}: An open source framework for applying targeted semantic changes, without degrading coherence.
  \item A \textbf{comprehensive measurement} of factors affecting model decisions under knowledge conflicts, including training methods, model size, model type, domain similarity, and characteristics of the substituted answer.
  \item \textbf{Practical guidance} on tailoring models to different desirable patterns of behaviour.
\end{itemize}

We hope our findings inform practitioners of the likely unexpected behaviours of their own models, and provides guidance on mitigating unwanted behaviour in favour of more generalizable, robust, and time-sensitive models.
Further, we encourage researchers to investigate more diverse forms of knowledge conflicts and adversarial substitutions with the aid of our open source framework.
